Scalable Algorithms for Learning High-Dimensional Linear Mixed Models

Linear mixed models (LMMs) are used extensively to model dependecies of observations in linear regression and are used extensively in many application areas. Parameter estimation for LMMs can be computationally prohibitive on big data. State-of-the-art learning algorithms require computational complexity which depends at least linearly on the dimension $p$ of the covariates, and often use heuristics that do not offer theoretical guarantees. We present scalable algorithms for learning high-dimensional LMMs with sublinear computational complexity dependence on $p$. Key to our approach are novel dual estimators which use only kernel functions of the data, and fast computational techniques based on the subsampled randomized Hadamard transform. We provide theoretical guarantees for our learning algorithms, demonstrating the robustness of parameter estimation. Finally, we complement the theory with experiments on large synthetic and real data.

==> synth.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.952in,
height=3.897in,
at={(0.521in,0.305in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Correlation},
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={at={(0.237,0.933)}, anchor=south west, legend columns=3, legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}

\begin{axis}[%
width=1.938in,
height=1.485in,
at={(3.303in,0.479in)},
scale only axis,
bar shift auto,
log origin=infty,
xmin=-4.71428571428571,
xmax=59.7142857142857,
xtick={ 5, 25, 50},
xlabel style={font=\color{white!15!black}},
xlabel={p},
ymin=0.95,
ymax=1.01,
axis background/.style={fill=white},
legend style={at={(0.237,0.933)}, anchor=south west, legend columns=3, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=4.571, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
5	0.996929705157476\\
25	0.993267019030926\\
50	0.999075672617928\\
};
\addplot[ybar, bar width=4.571, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
5	0.996954363564158\\
25	0.993267360202117\\
50	0.999064645549479\\
};
\end{axis}

\begin{axis}[%
width=1.938in,
height=1.481in,
at={(0.753in,0.484in)},
scale only axis,
bar shift auto,
log origin=infty,
xmin=-4.71428571428571,
xmax=59.7142857142857,
xtick={ 5, 25, 50},
xlabel style={font=\color{white!15!black}},
xlabel={p},
ymin=0.95,
ymax=1.01,
ylabel style={font=\color{white!15!black}},
ylabel={${\text{\it{} m = 10}}$},
axis background/.style={fill=white},
legend style={at={(0.237,0.933)}, anchor=south west, legend columns=3, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=4.571, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
5	0.997652698833161\\
25	0.999101627761055\\
50	0.993897066735141\\
};
\addplot[ybar, bar width=4.571, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
5	0.997630939579715\\
25	0.999097432217877\\
50	0.993854775458113\\
};
\end{axis}

\begin{axis}[%
width=1.938in,
height=1.481in,
at={(3.303in,2.547in)},
scale only axis,
bar shift auto,
log origin=infty,
xmin=-4.77777777777778,
xmax=59.7777777777778,
xtick={ 5, 25, 50},
ymin=0.95,
ymax=1.01,
axis background/.style={fill=white},
legend style={at={(0.237,0.933)}, anchor=south west, legend columns=3, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=3.556, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
5	0.998574472839469\\
25	0.994792187326547\\
50	0.994207708025963\\
};
\addlegendentry{arLMM-EM}

\addplot[ybar, bar width=3.556, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
5	0.99877415538049\\
25	0.994711615860887\\
50	0.994535320064633\\
};
\addlegendentry{REML}

\addplot[ybar, bar width=3.556, fill=mycolor3, draw=black, area legend] table[row sep=crcr] {%
5	0.999830186234127\\
25	0.9926\\
50	0.993017096760009\\
};
\addlegendentry{arLMM-AVC}

\node[below, align=center]
at (rel axis cs:0.5,1) {${\text{\it{} d = 25}}$};
\end{axis}

\begin{axis}[%
width=1.938in,
height=1.481in,
at={(0.753in,2.547in)},
scale only axis,
bar shift auto,
log origin=infty,
xmin=-4.77777777777778,
xmax=59.7777777777778,
xtick={ 5, 25, 50},
ymin=0.95,
ymax=1.01,
ylabel style={font=\color{white!15!black}},
ylabel={${\text{\it{} m = 1}}$},
axis background/.style={fill=white},
legend style={at={(0.237,0.933)}, anchor=south west, legend columns=3, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=3.556, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
5	0.999966178124274\\
25	0.998931391564688\\
50	0.999700980023756\\
};
\addplot[ybar, bar width=3.556, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
5	0.999968107020833\\
25	0.998942447956612\\
50	0.999699303354835\\
};
\addplot[ybar, bar width=3.556, fill=mycolor3, draw=black, area legend] table[row sep=crcr] {%
5	0.999983197508705\\
25	0.998934815984167\\
50	0.996610962732728\\
};
\node[below, align=center]
at (rel axis cs:0.5,1) {${\text{\it{} d = 5}}$};
\end{axis}
\end{tikzpicture}%
